Snap-Stabilizing Tasks in Anonymous Networks

We consider snap-stabilizing algorithms in anonymous networks. Self-stabilizing algorithms are well known fault tolerant algorithms : a self-stabilizing algorithm will eventually recover from arbitrary transient faults. On the other hand, an algorithm is snap-stabilizing if it can withstand arbitrary initial values and immediately satisfy its safety requirement. It is a subset of self-stabilizing algorithms. Distributed tasks that are solvable with self-stabilizing algorithms in anonymous networks have already been characterized by Boldi and Vigna in [BV02b]. In this paper, we show how the more demanding snap-stabilizing algorithms can be handled with standard tools for (not stabilizing) algorithms in anonymous networks. We give a characterization of which tasks are solvable by snap-stabilizing algorithms in anonymous networks. We also present a snap-stabilizing version of Mazurkiewicz' enumeration algorithm. This work exposes, from a task-equivalence point of view, the complete correspondence in anonymous networks between self or snap-stabilizing tasks and distributed tasks with various termination detection requirements.

==> vc.tex <==
\newcommand{\VCshash}{init-47-g0e9a636-dirty}
\newcommand{\VClhash}{0e9a636e75a40fd2741eae571b1b2f0d0045e6d0-dirty}
\newcommand{\VCauthname}{Emmanuel}
\newcommand{\VCauthemail}{emmanuel.godard@lif.univ-mrs.fr}
\newcommand{\VCauthsdate}{vendredi 27 avril 2018, 22:46:37 (UTC+0200)}
\newcommand{\VCauthidate}{2018-04-27}
\newcommand{\VCauthudate}{1524861997}
\newcommand{\VCcommname}{Emmanuel}
\newcommand{\VCcommemail}{emmanuel.godard@lif.univ-mrs.fr}
\newcommand{\VCcommsdate}{vendredi 27 avril 2018, 22:46:37 (UTC+0200)}
\newcommand{\VCcommidate}{2018-04-27}
\newcommand{\VCcommudate}{1524861997}
\newcommand{\VCrefnames}{redux}

